Extended Object Tracking Using Sets Of Trajectories with a PHD Filter

PHD filtering is a common and effective multiple object tracking (MOT) algorithm used in scenarios where the number of objects and their states are unknown. In scenarios where each object can generate multiple measurements per scan, some PHD filters can estimate the extent of the objects as well as their kinematic properties. Most of these approaches are, however, not able to inherently estimate trajectories and rely on ad-hoc methods, such as different labeling schemes, to build trajectories from the state estimates. This paper presents a Gamma Gaussian inverse Wishart mixture PHD filter that can directly estimate sets of trajectories of extended targets by expanding previous research on tracking sets of trajectories for point source objects to handle extended objects. The new filter is compared to an existing extended PHD filter that uses a labeling scheme to build trajectories, and it is shown that the new filter can estimate object trajectories more reliably.

==> include/backmatter/Back_cover.tex <==

\begin{titlepage}
\newgeometry{top=3cm, bottom=3cm,
			left=2.25 cm, right=2.25cm}	% Temporarily change margins		
\AddToShipoutPicture*{\backgroundpic{-4}{56.7}{figure/auxiliary/backpage_test.pdf}}
\addtolength{\voffset}{2cm}
\mbox{} 
\vfill
\end{titlepage}

==> include/frontmatter/Abstract.tex <==
% CREATED BY DAVID FRISK, 2018
Extended Object Tracking Using Sets of Trajectories with a PHD Filter\\
A Gamma Gaussian Inverse Wishart Trajectory PHD Filter with Smoothed Extent Estimates\\
Martin Marcusson, Jakob Sjudin\\
Department of Electrical Engineering\\
Chalmers University of Technology \setlength{\parskip}{0.5cm}

\thispagestyle{plain}			% Supress header 
% \setlength{\parskip}{0pt plus 1.0pt}
\section*{Abstract}
% It is becoming increasingly common to employ the help of automated systems to assist humans in tasks such as driving. 

An important part of many automated systems today is to estimate where surrounding objects are located. To do this, different tracking algorithms can be used to gain more accurate estimates from noisy sensor measurements over time. Due to increased sensor resolution, it is becoming more common that multiple measurements can originate from the same object at each scan. If this is the case, the object is often referred to as an extended object. This introduces new challenges but allows for the estimation of an objects size and shape. Additionally, questions related to the history of an objects state can be of interest in tracking. For example, what is the probability that an object was at a certain position in the past given the current position. Thus, the trajectory of an object is needed. Previously, many filters used for \acrfull{EOT} have not been able to reliably build trajectories. 

This thesis proposes a new \acrfull{PHD} filter used for \acrshort{EOT} that is able to build trajectories which also include estimates of the object's size and shape. The new filter is called the \acrfull{GGIWTPHD} filter and has been developed with a heuristic approach extending previous work. This is done by extending the \acrfull{GGIWPHD} filter by including results from the Trajectory PHD filter and introducing Bayesian smoothing of the extent estimates.

The performance of the \acrshort{GGIWTPHD} filter is evaluated by comparing it to a \acrshort{GGIWPHD} filter with labeled components using Monte Carlo simulation on simulated data. A metric is proposed for evaluating trajectories and is used to calculate a total \acrfull{RMS} error in each time step. It is shown that in situations with spatially close targets the trajectory estimates from the \acrshort{GGIWTPHD} filter are more accurate and reliable than trajectories built using estimates from a \acrshort{GGIWPHD} filter with labeled components. The GGIWTPHD is also shown to yield better extent and position estimates in all demonstrated scenarios.

% KEYWORDS (MAXIMUM 10 WORDS)
\vfill
Keywords: Multiple object tracking, Extended object, Gamma gaussian inverse wishart, Trajectories, Bayesian smoothing, Random finite sets, Probability hypothesis density, PHD filtering.

\newpage				% Create empty back of side
\thispagestyle{empty}
\mbox{}

==> include/frontmatter/Acknowledgements.tex <==
% CREATED BY DAVID FRISK, 2018
\thispagestyle{plain}			% Supress header
\section*{Acknowledgements}
We would like to thank Johan Degerman, SafeRadar Research AB who supervised the project and provided help when it was needed. We would also like to thank our examiner, Lars Hammarstrand who provided useful feedback throughout the project. Lastly, we would like to thank Lennart Svensson who provided support regarding some of the concepts dealt with in the thesis.

\vspace{1.5cm}
Martin Marcusson \& Jakob Sjudin, Gothenburg, June 2020 

\newpage				% Create empty back of side
\thispagestyle{empty}
\mbox{}

==> include/frontmatter/Glossary.tex <==
\makeglossaries

\newacronym{EOT}{EOT}{extended object tracking}
\newacronym{radar}{radar}{radio detection and ranging}
\newacronym{lidar}{lidar}{light detection and ranging}
\newacronym{MOT}{MOT}{multiple object tracking}
\newacronym{MEOT}{MEOT}{multiple extended object tracking}
\newacronym{DA}{DA}{data association}
\newacronym{RFS}{RFS}{random finite set}
\newacronym{PHD}{PHD}{probability hypothesis density}
\newacronym{GGIWPHD}{GGIWPHD}{Gamma Gaussian Inverse Wishart PHD}
\newacronym{GGIWTPHD}{GGIWTPHD}{Gamma Gaussian Inverse Wishart Trajectory PHD}
\newacronym{CT}{CT}{coordinated turn}
\newacronym{RMS}{RMS}{root mean square}
\newacronym{pdf}{pdf}{probability density function}

==> include/frontmatter/Titlepage.tex <==
% CREATED BY DAVID FRISK, 2018

% COVER PAGE
\begin{titlepage}
\newgeometry{top=3cm, bottom=3cm,
			left=2.25 cm, right=2.25cm}	% Temporarily change margins		
			
% Cover page background 
% \AddToShipoutPicture*{\backgroundpic{-4}{56.7}{figure/auxiliary/frontpage.pdf}}
\AddToShipoutPicture*{\backgroundpic{-4}{56.7}{figure/auxiliary/frontpage_test.pdf}}
\addtolength{\voffset}{2cm}

% Cover picture (replace with your own or delete)		
\begin{figure}[H]
\centering
\vspace{0cm}	% Adjust vertical spacing here
% \includegraphics[width=0.9\linewidth]{figure/Wind.png}
% \includegraphics[trim=550 150 500 150, clip, width=0.7\linewidth]{figure/front.pdf}
% \includegraphics[width=0.65\linewidth]{figure/crop.pdf}
\includegraphics[width=0.99\linewidth]{figure/front_crossingscenario.pdf}
\end{figure}

% Cover text Extended object tracking - A gamma gaussian inverse wishart trajectory probability hypothesis density filter
\mbox{} 
\vfill
\renewcommand{\familydefault}{\sfdefault} \normalfont % Set cover page fonthttps://www.overleaf.com/project/5e2e907b7196330001520d50
% \textbf{{\Huge 	Extended object tracking of large 	\\[0.2cm] 
%                 vehicles using medium range radar }} 	\\[0.5cm]
% \textbf{{\Huge 	Extended object tracking using sets of trajectories with a PHD filter \\[0.2cm]
%                 }} \\[0.2cm]
% {\Large A Gamma Gaussian Inverse Wishart Trajectory PHD filter with smoothed extent estimates}\\[0.5cm]
% Master's thesis in Systems, Control and Mechatronics \setlength{\parskip}{1cm}

% {\Large Martin Marcusson, Jakob Sjudin} \setlength{\parskip}{2.9cm}

% Department of Electrical Engineering \\
% \textsc{Chalmers University of Technology} \\
% Gothenburg, Sweden \the\year 

\renewcommand{\familydefault}{\rmdefault} \normalfont % Reset standard font
\end{titlepage}


% BACK OF COVER PAGE (BLANK PAGE)
\newpage
\restoregeometry
\thispagestyle{empty}
\mbox{}


% TITLE PAGE
\newpage
\thispagestyle{empty}
\begin{center}
	\textsc{\large Master's thesis \the\year}\\[4cm]		% Report number given by department 
	\textbf{\Large Extended Object Tracking Using Sets of Trajectories with a PHD Filter} \\[1cm]
	%\textbf{\Large Extended object tracking - A gamma gaussian inverse wishart trajectory probability hypothesis density filter} \\[1cm]
	{\large A Gamma Gaussian Inverse Wishart Trajectory PHD Filter with Smoothed Extent Estimates}\\[1cm]
	{\large Martin Marcusson}
	\\[0.2cm]
	{\large Jakob Sjudin}
	
	\vfill	
	% Logotype on titlepage	
	\begin{figure}[H]
	\centering
	% Remove the following line to remove the titlepage logotype
	\includegraphics[width=0.2\pdfpagewidth]{figure/auxiliary/logo_eng.pdf} \\	
	\end{figure}	\vspace{5mm}	
	
	Department of Electrical Engineering \\
	\emph{Division of Signal Processing and Biomedical Engineering}\\
	% Name of research group (if applicable)\\
	\textsc{Chalmers University of Technology} \\
	Gothenburg, Sweden \the\year \\
\end{center}


% IMPRINT PAGE (BACK OF TITLE PAGE)
\newpage
\thispagestyle{plain}
\vspace*{4.5cm}
Extended Object Tracking Using Sets of Trajectories with a PHD Filter\\
A Gamma Gaussian Inverse Wishart Trajectory PHD Filter with Smoothed Extent Estimates\\[0.2cm]
Martin Marcusson \\[0.1cm] Jakob Sjudin \setlength{\parskip}{1cm}

\copyright ~ Martin Marcusson, Jakob Sjudin, \the\year. \setlength{\parskip}{1cm}

Supervisor: Johan Degerman, SafeRadar Research Sweden AB\\
Examiner: Lars Hammarstrand, Department of Electrical Engineering \setlength{\parskip}{1cm}

Master's Thesis \the\year\\	% Report number given by department 
Department of Electrical Engineering\\
Division of Signal Processing and Biomedical Engineering\\
% Name of research group (if applicable)\\
Chalmers University of Technology\\
SE-412 96 Gothenburg\\
Telephone +46 31 772 1000 \setlength{\parskip}{0.5cm}

\vfill
% Caption for cover page figure if used, possibly with reference to further information in the report
Cover: A scenario where two objects cross paths, they start in the left and move to the right. Blue represents ground truth and the black dots are measurements. GGIWPHD filter estimates are red and GGIWTPHD filter estimates are green, where full lines are trajectories and dashed lines are estimated extent. Note that this scenario is not realistic, but it shows the capabilities of estimating trajectories with the GGIWTPHD filter. \setlength{\parskip}{0.5cm}

Typeset in \LaTeX \tagtemp\\
% Printed by Chalmers Reproservice\\
Gothenburg, Sweden \the\year



==> include/settings/Settings.tex <==
% CREATED BY DAVID FRISK, 2018

% BASIC SETTINGS
\usepackage{moreverb}								% List settings
\usepackage{textcomp}								% Fonts, symbols etc.
\usepackage{lmodern}								% Latin modern font
\usepackage{helvet}									% Enables font switching
\usepackage[T1]{fontenc}							% Output settings
\usepackage[english]{babel}							% Language settings
\usepackage[utf8]{inputenc}							% Input settings
\usepackage{amsmath}								% Mathematical expressions (American mathematical society)
\usepackage{amssymb}								% Mathematical symbols (American mathematical society)
\usepackage{graphicx}								% Figures
\usepackage{subfig}									% Enables subfigures
\usepackage{placeins}
\usepackage[backend=biber, style=numeric, sorting=none]{biblatex}
\numberwithin{equation}{chapter}					% Numbering order for equations
\numberwithin{figure}{chapter}						% Numbering order for figures
\numberwithin{table}{chapter}						% Numbering order for tables
\usepackage{listings}								% Enables source code listings
\usepackage{chemfig}								% Chemical structures
\usepackage[top=3cm, bottom=3cm,
			inner=3cm, outer=3cm]{geometry}			% Page margin lengths			
\usepackage{eso-pic}								% Create cover page background
\newcommand{\backgroundpic}[3]{
	\put(#1,#2){
	\parbox[b][\paperheight]{\paperwidth}{
	\centering
	\includegraphics[width=\paperwidth,height=\paperheight,keepaspectratio]{#3}}}}
\usepackage{float} 									% Enables object position enforcement using [H]
\usepackage{parskip}								% Enables vertical spaces correctly 
\usepackage{svg}
\usepackage{wrapfig}
\usepackage{algorithm}
\usepackage{algorithmic}
\usepackage{enumitem}
\usepackage{booktabs,siunitx}
\usepackage{longtable}
\usepackage{tikz}
\usetikzlibrary{shapes.geometric, arrows}

\usepackage{nextpage}

\usepackage[acronym,toc,nonumberlist,nopostdot,nogroupskip]{glossaries}
\setglossarystyle{listdotted}
\setlength{\glslistdottedwidth}{.3\linewidth}

% \setacronymstyle{long-short}

\addbibresource{include/backmatter/refs.bib}


% OPTIONAL SETTINGS (DELETE OR COMMENT TO SUPRESS)

% Disable automatic indentation (equal to using \noindent)
\setlength{\parindent}{0cm}                         

% Caption settings (aligned left with bold name)
\usepackage[labelfont=bf, textfont=normal,
			justification=justified,
			singlelinecheck=false]{caption} 		

		  	
% Activate clickable links in table of contents  	
\usepackage{hyperref}								
\hypersetup{colorlinks, citecolor=black,
   		 	filecolor=black, linkcolor=black,
    		urlcolor=black}


% Define the number of section levels to be included in the t.o.c. and numbered	(3 is default)	
\setcounter{tocdepth}{5}							
\setcounter{secnumdepth}{5}	


% Chapter title settings
\usepackage{titlesec}		
\titleformat{\chapter}[display]
  {\Huge\bfseries\filcenter}
  {{\fontsize{50pt}{1em}\vspace{-4.2ex}\selectfont \textnormal{\thechapter}}}{1ex}{}[]


% Header and footer settings (Select TWOSIDE or ONESIDE layout below)
\usepackage{fancyhdr}								
\pagestyle{fancy}  
\renewcommand{\chaptermark}[1]{\markboth{\thechapter.\space#1}{}} 


% Select one-sided (1) or two-sided (2) page numbering
\def\layout{2}	% Choose 1 for one-sided or 2 for two-sided layout
% Conditional expression based on the layout choice
\ifnum\layout=2	% Two-sided
    \fancyhf{}			 						
	\fancyhead[LE,RO]{\nouppercase{ \leftmark}}
	\fancyfoot[LE,RO]{\thepage}
	\fancypagestyle{plain}{			% Redefine the plain page style
	\fancyhf{}
	\renewcommand{\headrulewidth}{0pt} 		
	\fancyfoot[LE,RO]{\thepage}}	
\else			% One-sided  	
  	\fancyhf{}					
	\fancyhead[C]{\nouppercase{ \leftmark}}
	\fancyfoot[C]{\thepage}
\fi



% Enable To-do notes
\usepackage[textsize=tiny]{todonotes}   % Include the option "disable" to hide all notes
\setlength{\marginparwidth}{2.5cm} 


% Supress warning from Texmaker about headheight
\setlength{\headheight}{15pt}		


% Tag command (invisible)
\newcommand{\tagtemp}{\textcolor{white}{, template by David Frisk}}




